Color Deconvolution applied to Domain Adaptation in HER2 histopathological images

Breast cancer early detection is crucial for improving patient outcomes. The Institut Catal\`a de la Salut (ICS) has launched the DigiPatICS project to develop and implement artificial intelligence algorithms to assist with the diagnosis of cancer. In this paper, we propose a new approach for facing the color normalization problem in HER2-stained histopathological images of breast cancer tissue, posed as an style transfer problem. We combine the Color Deconvolution technique with the Pix2Pix GAN network to present a novel approach to correct the color variations between different HER2 stain brands. Our approach focuses on maintaining the HER2 score of the cells in the transformed images, which is crucial for the HER2 analysis. Results demonstrate that our final model outperforms the state-of-the-art image style transfer methods in maintaining the cell classes in the transformed images and is as effective as them in generating realistic images.

==> sections/conclusion.tex <==
\section{Conclusions}\label{sec:conclusions}

In conclusion, this study proposed a novel approach to address the challenge of color variations between HER2-stained histopathological images from different domains. Our approach combined the Color Deconvolution technique and the Pix2Pix GAN network to perform a style transfer while maintaining the intensity of the membranes, which is crucial for maintaining the HER2 score of the image. The results showed that our approach outperforms the state-of-the-art models in maintaining the cell classes and replicate their results in generating realistic images.

Our approach presented a promising solution for the color normalization problem in HER2-stained histopathological images, and it has the potential to be useful in clinical settings for pathological image analysis. By being able to compute this translation between stain brands, the DigiPatICS project can now perform all the inference within a single, common model for all the different hospitals that use different HER2 stain brands. This means less effort is required in acquiring the data to train one model for each hospital, making our proposed approach a practical and effective solution for improving cancer diagnosis and treatment outcomes. 

Further research can explore the application of this approach in other types of histopathological images with color normalization challenges. Overall, this work contributes to the development of more accurate and efficient pathological image analysis tools, which could ultimately improve clinical decision-making and patient outcomes.
